TalkToModel: Explaining Machine Learning Models with Interactive Natural Language Conversations

Machine Learning (ML) models are increasingly used to make critical decisions in real-world applications, yet they have become more complex, making them harder to understand. To this end, researchers have proposed several techniques to explain model predictions. However, practitioners struggle to use these explainability techniques because they often do not know which one to choose and how to interpret the results of the explanations. In this work, we address these challenges by introducing TalkToModel: an interactive dialogue system for explaining machine learning models through conversations. Specifically, TalkToModel comprises of three key components: 1) a natural language interface for engaging in conversations, making ML model explainability highly accessible, 2) a dialogue engine that adapts to any tabular model and dataset, interprets natural language, maps it to appropriate explanations, and generates text responses, and 3) an execution component that constructs the explanations. We carried out extensive quantitative and human subject evaluations of TalkToModel. Overall, we found the conversational system understands user inputs on novel datasets and models with high accuracy, demonstrating the system's capacity to generalize to new situations. In real-world evaluations with humans, 73% of healthcare workers (e.g., doctors and nurses) agreed they would use TalkToModel over baseline point-and-click systems for explainability in a disease prediction task, and 85% of ML professionals agreed TalkToModel was easier to use for computing explanations. Our findings demonstrate that TalkToModel is more effective for model explainability than existing systems, introducing a new category of explainability tools for practitioners. Code & demo released here: https://github.com/dylan-slack/TalkToModel.

==> capabilites.tex <==
\begin{table*}[t]
    \tiny
    \centering
    \begin{tabular}{lllll}
        \toprule
        & \Centerstack[l]{\bf \parse{operation}, \args{arguments}, and description \\ \scriptsize \args{data} \textit{implicitly provided as first argument to operations}} & Example user \userinput{utterance} and \parse{parse} & \Centerstack[l]{\sys Response \\  \textcolor{blue}{\textbf{\texttt{[abb.]}}}: abbreviated for conciseness} \\
        \midrule
        \vspace{3mm} \multirow{14}{*}{\centering \rotatebox[origin=c]{90}{ Data}} & \Centerstack[l]{\parse{filter(}\args{feature, value, comparison}\parse{)}: \\filters data by feature, label, or prediction} & \Centerstack[l]{\userinput{What are the predictions on people older than 30?} \\ \parse{predict(filter(}\args{data, age, 30, >}\parse{))}} &  \scriptsize \sysresponse{
        \Centerstack[l]{\footnotesize On data with \textbf{age greater than 30.0}, the model predicts: \\ \footnotesize \quad\ding{233} \textbf{No Diabetes} on 46.8\% of data \\ \footnotesize \quad\ding{233} \textbf{Diabetes} on 53.2\% of data}} \\
        \vspace{3mm} & \Centerstack[l]{\parse{change(}\args{feature, value, variation}\parse{)}: \\ modifies data by increasing, decreasing, or\\setting a feature value} & \Centerstack[l]{\openui{If patient 22's BMI increases by 10, how likely are}\\ \closeui{they to have diabetes?} \\ \parse{likelihood(change(}\\\parse{filter(}\args{data, id, 22, =}\parse{)}\args{,} \args{bmi, 10, increase}\parse{))}} & \scriptsize\sysresponse{\Centerstack[l]{\footnotesize The model predicts \textbf{data id 22} with \textbf{bmi is increased by} \\ \footnotesize \textbf{10} as: \\ \footnotesize \quad\ding{233} \textbf{No Diabetes} with \textit{90.2\%} probability \\  \footnotesize \quad\ding{233} \textbf{Diabetes} with \textit{9.8\%} probability }} \\
        \vspace{3mm} & \parse{show(}\args{label}\parse{)}: show data or gold labels & \Centerstack[l]{\userinput{Show me patient id 102} \\ \parse{show(filter(}\args{data, id, 102, =}\parse{)}\args{, False}\parse{)}} & 
        
        \scriptsize\sysresponse{\Centerstack[l]{\footnotesize For \textbf{data id 102}, the features are: \\ \footnotesize\quad\ding{233} \textit{glucose}: 125 \\ \footnotesize\quad\ding{233} \textit{bmi}: 22.5  \myquad[15] \textcolor{blue}{\textbf{\texttt{[abb.]}}} }} \\
        
       \vspace{3mm} & \Centerstack[l]{\parse{statistic(}\args{metric, feature}\parse{)}: compute \\ summary statistics} & \Centerstack[l]{\userinput{What's the average age in the data}\\  \parse{statistic(}\args{mean, age}\parse{)}} & \sysresponse{\Centerstack[l]{\footnotesize Over \textbf{all the data}, the \textbf{average age} is: \textit{34.2}}\myquad[5]} \\
       \vspace{0.5mm} & \parse{count()}: count data & \Centerstack[l]{\openui{Count how many patients the model predicts to} \\ \closeui{have diabetes.} \\ \parse{count(filter(}\args{prediction, true, =}\parse{))}} & \scriptsize\sysresponse{\Centerstack[l]{\footnotesize There are \textbf{111 items} in the data where the model \\ \footnotesize predicts \textbf{Diabetes}}\myquad[4]} \\
        \vspace{0.5mm} & \parse{or(}\args{op1, op2}\parse{)}: logical ``or'' & \\
        \vspace{0.5mm} & \parse{and(}\args{op1, op2}\parse{)}: logical ``and'' & \\
        \midrule
        \vspace{0.5mm} \multirow{5}{*}{\centering \rotatebox[origin=c]{90}{Explainability}} & \shortstack[l]{\parse{explain(}\args{method}\parse{)}: computes feature \\ importances} &  \\
         \vspace{0.5mm} & \parse{cfe()}: counterfactual explanations & \\
         \vspace{0.5mm} & \parse{topk(}\args{k}\parse{)}: top k most important features & \\
         \vspace{0.5mm} & \shortstack[l]{\parse{interaction()}: interactions between\\features} & \\
         \vspace{0.5mm} & \shortstack[l]{\parse{mistakes()}: summarize common patterns \\ in mistakes} &  \\
        \midrule
        \vspace{0.5mm} \multirow{3}{*}{\centering \rotatebox[origin=c]{90}{ML}} & \parse{predict()}: predictions \\
        \vspace{0.5mm} & \parse{likelihood()}: class probabilities \\
        \vspace{0.5mm} & \parse{score(}\args{metric}\parse{)}: performance metrics \\
        \midrule
        \vspace{0.5mm} \multirow{2}{*}{\rotatebox[origin=c]{90}{Conv.}} & \parse{previousfilter()}: get last filter \\
        \vspace{0.5mm} & \parse{previousoperation()}: get last operation \\
        \midrule
        \vspace{0.5mm} \multirow{4}{*}{\centering \rotatebox[origin=c]{90}{Description}} & \parse{function()}: describe system capabilities &  \\
        \vspace{0.5mm} & \parse{data()}: summarize dataset & \\
        \vspace{0.5mm} & \parse{model()}: describe model & \\
        \vspace{0.5mm} & \parse{define(}\args{term}\parse{)}: define term & \\
        \bottomrule
    \end{tabular}
    \caption{\bf Capabilities (dylan working on this...)}
    \label{tab:na}
\end{table*}

==> relwork.tex <==
\section{Related Work}


In this section, we contextualize our work in the related work of explainability and interactive systems.
In particular, we describe how researchers have developed explanations in order to help model stakeholders understand the predictions of state of the art machine learning models, which have become increasingly complex over the last few decades.

\paragraph{Explanation Techniques} 

Machine learning models have increasingly been applied to high-stakes settings that significantly impact people's lives, including disease prediction, parole decisions, and environmental prediction~\cite{sacair, compas, Uddin2019}.
Yet, many machine learning models' internal workings are not easily understood, making it difficult to trust their predictions in these rather impactful settings.
These \textit{black-box} models include deep decision trees or neural networks, and people generally have difficulty understanding the reasons for their predictions~\cite{Slack2019AssessingTL}.
Consequently, practitioners have often turned to \textit{inherently interpretable} machine learning models for these applications, which people can more easily understand.
There exist several methods in the literature that learn inherently interpretable models, such as decision list and sets \cite{lakkaraju2016interpretable, angelino2017learning, ustunSuperSparse2016, zengRecid2015}, prototype based models \cite{Shin_Kim_Yoon_Shin_2022, ChenEtAl2019, Hase2019InterpretableIR} and generated additive models \cite{lou2013accurate, NEURIPS2021_251bd044, chang2021node, chang2021interpretable, zhangaxiomatic}. 

However, black-box models are often more flexible and accurate, motivating the development of \textit{post-hoc} explanations that explain the predictions of trained ML models~\cite{lime:whi16, slackreliable21, gradcam, slack2021defuse, Ribeiro_Singh_Guestrin_2018, oodhase2021}.
To this end, several methods have been proposed that generate post-hoc explanations for complex, black-box models.
Some of the most commonly used post hoc explanation methods are the feature attribution methods LIME~\cite{ribeiro2016should} and SHAP~\cite{lundberg2017unified}, which train linear models that capture the local region around a prediction with high fidelity. 
There also exists explanation methods that use internal details such as gradient access to highlight important features for model predictions~\cite{Simonyan14a, smilkov2017smoothgrad, sundararajanAxiomaticAttribution2017}.

While explanation methods are useful tools for understanding models, there are also several works that evaluate their limitations.
For example, multiple works demonstrate explanations can be inconsistent and unstable~\cite{Ghorbani_Abid_Zou_2019, AlvarezMelis2018OnTR, slackreliable21, zafar-etal-2021-lack}.
Further techniques show how explanations can be attacked by adversaries, demonstrating they can be unreliable in adversarial scenarios and can mask undesirable aspects of the model~\cite{SlackHilgard2020FoolingLIMESHAP, manipcfes:neurips21, liuAdvAttacks2021}.
Finally, additional works demonstrate explanations may be unfair towards certain groups in the data for complex, non-linear models~\cite{daifairness22, balagopalan22}.


\paragraph{Interactive Explanation Methods} 
While most explanation methods are designed to generate a single explanation for a prediction, there are a few works that consider generating explanations in an interactive manner.
These include dashboard techniques, such as the Language Interpretability Tool (LiT)~\cite{tenney2020language}, which is designed to understand natural language processing (NLP) models and the "What-If" Tool~\cite{whatif}, which is aimed at performing what if analyses for models. 
While these tools provide useful ways for engaging models, they do not automatically map user intentions to analyses, provide focused responses, and engage in natural language dialogues, which we find is critical for semi-technical domain experts to understand ML models.
In addition, these techniques are limited to specific model types and analyses, while \sys supports a much broader scope of techniques.

In addition, there exist works that motivate dialogue based explanations.
For instance, Glassbox \cite{sokol2018glass} provides an outline for a prototype system where users provide language queries and receive counterfactual explanations for decision trees, and they propose demonstrating the system on a loan application setting.
Further works propose building language interfaces for explanations.
For example, \citet{feldhus2022mediators} propose desiderata for dialogue based explanations for sentiment analysis models. 
In addition, \citet{lakkaraju2022rethinking} interview domain experts, find they strongly desire open ended dialogues for understanding models, and propose desiderata and technical considerations for such systems.
Overall, these works provide useful outlines and desiderata for developing open ended dialogues for explaining models.



==> semistructured.tex <==
While in the previous section we evaluated the capabilities of \sys in a controlled setting, we also wanted to evaluate whether \sys can deliver value to domain experts who are stakeholders in ML models in a real world setting.
To this end, we approached operations team at an AI health insurance company that uses ML to analyze large amount of healthcare claims data for fraud and waste detection to conduct a semi-structured interview using \sys.
The operations team is responsible for ensuring the company's ML models lead to business success, and they must be capable of understanding why their models make predictions and whether to trust model outcomes, though they may have minimal or no formal ML background.

In order to evaluate whether \sys could deliver value in this setting, we invited the head of the operations team to a \sys session lasting around $4$ hours.
Because their models are proprietary, we instead provided \sys using the Diabetes dataset because of their experience with medical oriented domains.
We initially asked them about difficulties that arise using ML as someone who works in operations.
They indicated their largest issues arise from communication between operations and data scientists, and they had some experience with feature importance explanations.
In particular, their issues can arise both from operations struggling to understand which features models are considering and how they work in general, affecting their capacity to serve customer needs.
On the other hand, data scientists sometimes fail to understand critical health insurance domain knowledge, affecting their ability to produce business useful models.
Next, we provided an overview of the scope of the system and what types of questions they could expect the system to answer.
We then let them explore \sys in an open ended manner and encouraged them to think out loud as they did.
Because they did not have access to a desktop computer for the entirety of the interview, we asked them to dictate the questions, and we typed them in to \sys over a shared screen. 
During this time, they constructed $36$ questions for the system.
Most of these questions were about prediction probabilities for specific patients, feature importance explanations, and the distribution of different predictions.
For example, ``for patient 237 what are the most important indicators for them being predicted by the model'' and ``what is the average age of people who are predicted likely to have diabetes by the model.''
Because they did not ask complex filtering questions or compositional questions the parsing accuracy was relatively highly failing just $3/36$ questions (accuracy rate $92\%$).
During this time, most of their comments were about surprising things things they found in the data using \sys.
For instance, they expressed surprise that the \texttt{insulin} feature is not an important feature for the model and about the relationship between the \texttt{glucose} and \texttt{insulin} levels and whether someone had diabetes.
They were excited that they could quickly figure out that the model did not align with their own mental image of diabetes prediction and brain stormed several additional features that could be included in the dataset to help improve model performance.
However, they expressed skepticism at certain parts of the system when it could not answer questions about the prediction task such as ``do you predict diabetes type 1.'' 
Finally, we asked them about their overall feedback on \sys.
They expressed that the \sys interface is highly useful for model understanding. They indicated they really liked the fact that using \sys felt like a quick and easy personal interaction instead of a tedious process writing many SQL queries to get results.
They also expressed that interface worked quite well overall stating ``the interface is awesome'' and ``really fun to use.''
Last, they asked that we notify them for future releases of the software and brainstormed several ways to integrate it into existing tools, including as a Microsoft Outlook add-on.
Though they expressed \sys was quite useful for understanding models, they also indicated it could be improved in a few ways. First, they felt high level performance metrics, feature definitions, and aggregate feature importances should be printed out in a report shown ahead of the time before using the system because typing these in repeatedly is a bit tiresome.
In addition, they wanted to know more about why the model is uncertain on different inputs and felt that the feature importance measures included in \sys could be improve to help answer this question.

==> titlepage.tex <==
\onecolumn

 \begin{center}
\textbf{Title}\\
TalkToModel: Understanding Machine Learning Models With Open-Ended Dialogues \\

\hspace{10pt}

\textbf{Author Line}\\
Dylan Slack$^a$, Satyapriya Krishna$^b$, Himabindu Lakkaraju$^{1b}$, Sameer Singh$^{1ac}$ \\

\hspace{10pt}

$a$) Department of Computer Science \\
     University of California, Irvine \\
     Irvine, CA 92697 \\
\vspace{5pt}
$b$) Department of Computer Science \\
     Harvard University \\
     Cambridge, MA 02138 \\
\vspace{5pt}
$c$) Allen Institute for Artificial Intelligence \\
     Seattle, WA 98103 \\
\vspace{5pt}
$1$) Equal Contribution \\
\vspace{5pt}

\vspace{10pt}
\textbf{Corresponding Author}\\
\vspace{3pt}
Dylan Slack \\
274 Sandcastle, Aliso Viejo, CA 92656 \\
415-847-2440 \\
\texttt{dslack@uci.edu}

\vspace{10pt}
\textbf{Preprint Server}\\
\vspace{3pt}
Deposited to arXiv at \texttt{https://arxiv.org/abs/2207.04154} under Non-exclusive license to distribute

\vspace{10pt}
\textbf{Classification}\\
\vspace{3pt}
Major: Physical \\
Minor: Computer Sciences \\

\vspace{10pt}
\textbf{Keywords}\\
\vspace{3pt}
Machine Learning, Explanations, Dialogues


\vspace{10pt}


\end{center}


\twocolumn
